Beyond Model Collapse: Scaling Up with Synthesized Data Requires Verification

Large Language Models (LLM) are increasingly trained on data generated by other LLM, either because generated text and images become part of the pre-training corpus, or because synthetized data is used as a replacement for expensive human-annotation. This raises concerns about \emph{model collapse}, a drop in model performance when their training sets include generated data. Considering that it is easier for both humans and machines to tell between good and bad examples than to generate high-quality samples, we investigate the use of verification on synthesized data to prevent model collapse. We provide a theoretical characterization using Gaussian mixtures, linear classifiers, and linear verifiers to derive conditions with measurable proxies to assess whether the verifier can effectively select synthesized data that leads to optimal performance. We experiment with two practical tasks -- computing matrix eigenvalues with transformers and news summarization with LLMs -- which both exhibit model collapse when trained on generated data, and show that verifiers, even imperfect ones, can indeed be harnessed to prevent model collapse and that our proposed proxy measure strongly correlates with performance.

==> base/10_broader_impact.tex <==
\section{Broader Impact}\label{sec:impact}

{The study explores the use of synthesized data from generative models as a cost-effective alternative to human-labeled data, aiming to address concerns about model collapse where performance degrades despite increased data volumes. By investigating data selection through reinforcement, the study theoretically and empirically demonstrates that human or oracle supervision can enhance the quality of synthesized datasets, preventing model collapse and potentially surpassing the original dataset's performance. This approach holds significant social impact by proposing a scalable, efficient method to leverage AI-generated data across various domains, reducing dependency on extensive human labeling efforts and mitigating the risks associated with iterative training on synthesized data. The reinforcement-guided data selection can foster more robust and reliable AI models, ultimately contributing to advancements in diverse fields such as language processing, image recognition, and beyond. However, this method also introduces potential negative social impacts. If the verifier, crucial for distinguishing high-quality from low-quality synthesized data, is compromised, it could lead to the propagation of erroneous or malicious data throughout the model. Such vulnerabilities could be exploited through poisoning or targeted attacks, resulting in significant biases, misinformation, and harmful outcomes in AI-driven decisions, particularly in sensitive sectors like healthcare, finance, and law enforcement. Moreover, the reliance on synthesized data could amplify existing biases, reduce cultural and cognitive diversity, and erode public trust in AI technologies, increasing societal vulnerabilities to cyber threats and compromising the perceived reliability and fairness of AI systems.}

==> base/8_theory_append.tex <==
\section{A General Theory of Pruning}\label{app:theory}




\textbf{Condition for High-dimensional Limit.} Consider a probability distribution $P$ over $\mathbb R^d \times \{0,1\}$ with the following high-dimensional property
\begin{mdframed}
\begin{condition}
\label{cond:main}
Given $N \le N(d)$ iid samples $(x_1,y_1),\ldots,(x_N,y_N)$ from $P$ with $N \le N(d)$, the following hold estimates w.p $1-o(1)$ uniformly on all $i,j \in [N]$, in the limit $d \to \infty$
\begin{align}
    \|x_i\|^2 &\simeq 1\label{eq:unit-norm},\\
    x_i^\top x_j &\simeq \begin{cases}
        a,&\mbox{ if }y_i = y_j,\\
    b,&\mbox{ if }y_i \ne y_j\label{eq:cross-class-cor},
    \end{cases}
\end{align}
where $b < a < 1$ are constants. For simplicity of presentation of our results, We will further assume that $b=-a$ or $b=0$.
\end{condition}
\end{mdframed}
The above structural condition is inspired by an assumption in \cite{das2023understanding}.

In the Gaussian Mixture example in Section \ref{subsec:3.1}, we may take
\begin{eqnarray}
a=\|\mu\|^2,\quad b= -a. 
\end{eqnarray}
Condition \ref{cond:main} then holds thanks to concentration, with $N(d) = e^{\Theta(d)}$.


\begin{remark}
    Note that the parametrization $(\phi,\psi)$ and $(p_{00},p_{11})$ describe the same RLHF-type policy via the following bijective transformation.
    \begin{align}
        p_{00} &= p_{11} = (1-p)\phi/2,\quad p_{01}=p_{10} = 
 p \psi /2.
    \end{align}
\end{remark}

\bbb{
For Gaussian mixture distribution $P$ with isotropic covariance, we have
$$
p_{00} = p_{11} = \mathbb P(x^\top w_p > 0,\, x^\top w_g > 0 \mid y=1)\mathbb P(y=1) = \mathbb P(z_p >-\mu^\top w_p,\,z_g >-\mu^\top w_g)/2,
$$
where $(x,y) \sim P$, so that the distribution of $x$ conditioned on $y=1$ is $N(\mu, \Sigma)$ with $\Sigma=I_d$; $z_g:=z^\top w_g$ and $z_p:=z^\top w_p$, for $z \sim N(0,\Sigma)$.
Now, assume WLOG that $\|w_g\|=\|w_p\|=1$, and observe that $(z_g,z_p)$ is bivariate normal with variance $\sigma^2=1$ and correlation coefficient $\rho=w_p^\top w_g$. The joint pdf is thus
$$
f(u,v) = \frac{1}{2\pi\Delta}e^{-\frac{1}{2\Delta^2}(u^2+v^2-2\rho u v)} = \frac{1}{\sqrt{2\pi\Delta^2}}e^{-\frac{1}{2\Delta^2}(v-\rho u)^2}\frac{1}{\sqrt{2\pi}}e^{-u^2/2},
$$
where $\Delta=\sqrt{1-\rho^2}$. We deduce that
\begin{align*}
   2 p_{00} &= \int_{-\mu^\top w_g}^\infty \left(\int_{-\mu^\top w_p}^\infty \frac{1}{\sqrt{2\pi\Delta^2}}e^{-\frac{1}{2\Delta^2}(v-\rho u)^2}\mathrm dv\right)\varphi(u)\mathrm du\\
    &= \int_{-\mu^\top w_g}^\infty\Phi\left(\frac{\rho u+\mu^\top w_p}{\Delta}\right)\varphi(u)\mathrm du\\
    &= \int_0^\infty \Phi\left(\frac{\rho (u + \mu^\top w_g) + \mu^\top w_p}{\Delta}\right)\varphi(u+\mu^\top w_g)\mathrm du.
\end{align*}
One can derive similar expressions for $p_{01}=p_{10}$,
namely
\begin{align*}
2p_{01} = \int_0^\infty \Phi\left(\frac{\rho (u - \mu^\top w_g) - \mu^\top w_p}{\Delta}\right)\varphi(u-\mu^\top w_g)\mathrm du.
\end{align*}}

\begin{figure}[!htb]
    \centering
        \includegraphics[width=.45\textwidth]{RLHF.png}
        % \includegraphics[width=.43\textwidth]{thresholds.png}
    % \includegraphics[width=.45\textwidth]
    % {prune.png}
   \caption{\textbf{Empirical Confirmation of Theorem \ref{thm:main}.} Comparing the breakdown points of different models. Here, the task is classifying a Gaussian mixture, with infinite training samples from datasets generated from a model with classification error rate $p$ (x-axis). Notice the sharp phrase-transitions where the model suddenly switches from perfect accuracy to worse-than-chance, a phenomenon predicted by Theorem \ref{thm:main}. % \textbf{Top Right.} "SD" stands for self-distillation, and "xn" means iterative self-distilling the same model $n$ times. Notice how a model pruning with a teacher's margin is already stronger than a few distillations (here it seems to actually matches double-distillation), and much stronger than the original student. Also notice how repeated self-distillation approaches RLHF. 
    Comparing $p_{up}$, approximated with $\sup\{p \mid acc(\widehat f_N) \ge 90\%\}$ (computed empirically), against the analytic estimate $p^-_\star(t)$ given in \ref{thm:main} (for $t=0.1$). Again, the results are in excellent agreement with the predictions of Theorem \ref{thm:main}. 
    % Even for $p > 1/2$, notice how the models with $\psi/\phi<1$ still continue to perhaps above chance level ($50\%$ accuracy). % \textbf{Bottom.} Comparing with margin-based pruning strategies. Again, notice the sharp phrase-transitions predicted by Theorem \ref{thm:main}.
    }
    \label{fig:curve_append}
\end{figure}

% The thresholds $p^\pm_\star(t)$ appearing in the above theorem is are proxies for the so-called \emph{breakdown points} $p_{up} \ge p_{down}$ defined by
% \begin{align}
%     p_{up} &= \inf\left\{p \in [0,1] \,\big|\, acc(\widehat f_N) \overset{a.s}\to 0\%\text{ in the limit }N \to \infty\right\},\\
%         p_{down} &= \sup\left\{p \in [0,1] \,\big|\, acc(\widehat f_N) \overset{a.s}\to 100\%\text{ in the limit }N \to \infty\right\}.
% \end{align}
% Theorem \ref{thm:main} implies $p_{down} \ge p^-_\star(t)$ and $p_{up} \le p^+_\star(t)$ for all $t \in (0,1)$. Consequently,
% \begin{corollary}
%     Under the hypotheses of Theorem \ref{thm:main}, it holds that $p_{up} = p_{down}$.
% \end{corollary}
% \yunzhen{Do we need it?}


==> checklist.tex <==
\section*{NeurIPS Paper Checklist}



\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The abstract and introduction clearly state the contributions and the scope.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Limitations are discussed in the Discussion and Limitation Section \ref{sec:conc}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper provides the full set of assumption in Section \ref{subsec:3.1} and \ref{subsec:3.2} and a complete proof in Appendix \ref{sec:proof}. A proof sketch is provided in Section \ref{app:sketch}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The experimental sections provide comprehensive details to enable the reproduction of our results. Our key contribution lies in using these experiments to validate the theoretical findings. We utilize open-source datasets and open-source code to ensure transparency and reproducibility.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The code for the arithmetic task is available at \url{https://github.com/facebookresearch/LAWT} with the exact command we use. For the news summarization task, we use the open-source dataset available at \url{https://huggingface.co/datasets/csebuetnlp/xlsum}, utilizing the standard Hugging Face trainer, which can be found at \url{https://github.com/huggingface/transformers/blob/main/examples/pytorch/language-modeling/run_clm.py}. We provide all the hyperparameters we use to reproduce the script in Section \ref{sec:news_append}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All the details and provided in both the main text and the appendix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide error bars only for the simulation results within a 2-$\sigma$ range. Due to resource limitations, we are unable to provide error bars for the transformer and training with Llama-2. However, we believe that the differences in the metrics are already significant.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Compute resources are detailed alongside the experimental procedures in the Appendix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: There is no link can be used to identify the authors. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: In Section \ref{sec:impact}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper poses no such risks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We include the citation, code or dataset link, and license information in the Appendix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not release new assets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsorcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> hutter.tex <==

\section{Hutter with Label-Noise (half-baked WIP, consume at your own risk)}
Let $N,M \ge 2$ be integers, $\pi \in (0,1]$, and consider a probability distribution $P$ on $\mathbb N_* \times [M]$ given as follows
\begin{equation}
    x \sim Zipf(\beta),\quad y  \overset{D}{=} \begin{cases}
        f_0(x),&\mbox{ w.p }\pi,\\
        u,&\mbox{ w.p }1-\pi,
    \end{cases}
\end{equation}
where $u \sim U([M])$ is independent of $x$. Thus, conditioned on $x$, the distribution of $y$ is a mixture
\begin{equation}
    p(y \mid x) = \pi\delta_{f_0(x)}(y) + \frac{1-\pi}{M},
\end{equation}
of an atomic mass and a uniform distribution. Given a (possibly random) predictor $\hat f:\mathbb N_* \to [M]$, its test error $\err(\hat f)$ is defined by
\begin{equation}
    \err(\hat f) = \mathbb P_{x,y,\hat f}(\hat f(x) \ne y),\text{ for a random test point }(x,y) \sim P.
\end{equation}
Also, let $\err_* := \inf_{\hat f}\err(\hat f)$ by the Bayes-optimal error.
\begin{lemma}
    It holds that $\err_* = (1-1/M)(1-\pi)$. Thus, the Bayes error for the problem only vanishes in the limit $\pi \to 1$.
\end{lemma}
\begin{proof}
    Indeed, Thanks to Proposition 1 of \url{https://arxiv.org/abs/1712.00812}, one computes
    \begin{eqnarray*}
        \begin{split}
    \err_* &:= \inf_{\hat f}\err(\hat f) = 1-\sum_x p(x)\max_y p(y\mid x) = 1-\left(\pi + \frac{1-\pi}{M}\right) = (1-1/M)(1-\pi),
        \end{split}
    \end{eqnarray*}
    as claimed.
\end{proof}
\subsection{Learning}
Let $D_T = \{(x_1,y_1),\ldots,(x_T,y_T)\}$ be an iid sample of size $T$ from $P$. For any $(x,y) \in \mathbb N_* \times [M]$, define $n_T(x,y) := \sum_{t=1}^T 1_{(x_t,y_t) = (x,y)} \in [0,T]$ be the number of times $(x,y)$ appears in the sample $D_T$, and consider the model $\hat f_T:\mathbb N_* \to [M]$ defined by
\begin{eqnarray}
\hat f_T(x) := \max_y n_T(x,y),
\end{eqnarray}
with ties broken by an arbitrary rule. This predictor is nothing but a finite-sample estimate of the Bayes-optimal model
\begin{eqnarray}
f_*(x) = \arg\max_y p(x,y) = \arg\max_y p(y\mid x).
\end{eqnarray}
which attains the optimal test error $\err_*$. We have the following result.
 % In fact, one can show that
% $$
% 0 \le \err(\hat f_T) - \err_* \le \sum_x p(x)\operatorname{TV}(\hat p_T(\cdot\mid x),p(\cdot \mid x)) \le \frac{1}{2}\sqrt{\frac{M}{T}}.
% $$

\begin{theorem}
\label{thm:noisyhutter}
   Define $c:=1-1/\beta \in (0,1)$. For $\pi \ge C_0\log(M)/M$ and large $T$, it holds that
    \begin{eqnarray*}
        0 \le \err(\hat f_T) - \err_\star \lesssim (CT)^{-c},
    \end{eqnarray*}
    where $C > 0$ is a constant which only depends on $\pi$.
\end{theorem}
Thus, the extension of the Hutter model to include label noise doesn't provide any interesting new phenomena: it only adds an offset to usual scaling laws.

\subsection{Going Beyond Hutter}
Note that the function $f_0$ in Hutter model or the extension thereof presented in the previous section is nothing but the \emph{regression function} for the underlying joint distribution $P$ of $(x,y)$, i.e $f_0(x) = \arg\min_y P(y \mid x)$.
This means that one could more generally simply consider an arbitrary distribution $P$, and then define
\begin{eqnarray}
    f_P(x) := \arg\min_y P(y \mid x),
\end{eqnarray}
to play the role of $f_0$.

==> neurips_theory_safecopy.tex <==
\section{A General Theory of Pruning with Reinforcement}\label{app:theory}


In Section \ref{sec:theory_main_paper} we have presented a special case of our general theory, which we describe here in more generality and detail.

\subsection{Data Distribution} 
\julia{Note to self: remove some euqation numbers, redefine doubly defined labels}
Consider a probability distribution $P$ over $\mathbb R^d \times \{0,1\}$ with the following high-dimensional property
\begin{mdframed}
\begin{condition}
\label{cond:main}
Given $N \le N(d)$ iid samples $(x_1,y_1),\ldots,(x_N,y_N)$ from $P$ with $N \le N(d)$, the following hold estimates w.p $1-o(1)$ uniformly on all $i,j \in [N]$, in the limit $d \to \infty$
\begin{align}
    \|x_i\|^2 &\simeq 1\label{eq:unit-norm},\\
    x_i^\top x_j &\simeq \begin{cases}
        a,&\mbox{ if }y_i = y_j,\\
    b,&\mbox{ if }y_i \ne y_j\label{eq:cross-class-cor},
    \end{cases}
\end{align}
where $b < a < 1$ are constants. For simplicity of presentation of our results, We will further assume that $b=-a$ or $b=0$.
\end{condition}
\end{mdframed}
The above structural condition is inspired by an assumption in \cite{das2023understanding}.


% and proposed a self-distillation as a way to boost accuracy for certain values of the corruption parameter $p$.
For simplicity of exposition, we will only consider balanced distributions, meaning that
\begin{eqnarray}
\mathbb P(y=1) = \mathbb P(y=0) = 1/2,\text{ for }(x,y) \sim P.
\end{eqnarray}
% \begin{definition}
% \label{df:symmetric}
%     For any $w \in \mathbb R^d$, $m \in \mathbb R$, and $k \in \{0,1\}$, define  $P_k(w,m) \in [0,1]$ by
%     \begin{eqnarray}
%         P_k(w,m) := \mathbb P(x^\top w > m \mid y=k),\text{ where }(x,y) \sim P.
%         \label{eq:Pk}
%     \end{eqnarray}
%     This is the probability that a random test point $x \in \mathbb R^d$ sampled from class label $k$ lies in the half-space $x^\top w - m > 0$. 
    
%     If $P_0(w,m) \equiv P_1(-w,m)$, we say the underlying classification problem is symmetric.
% \end{definition}

\paragraph{Gaussian Mixture Example.}
As a first example, in the case of Gaussian mixtures where the features have conditional distribution given by
\begin{eqnarray}
x \mid y \sim N(\mu_y,\Sigma),\\
\end{eqnarray}
where $\mu_y = (2y-1)\mu$, for some $\mu \in \mathbb R^d$ and positive-definite matrix $\Sigma$ with $\mathbb E\,\|x\|^2 = \|\mu\|^2+\operatorname{tr}\Sigma = 1$, we may take
\begin{eqnarray}
a=\|\mu\|^2,\quad b= -a. 
\end{eqnarray}
Condition \ref{cond:main} then holds thanks to concentration, with $N(d) = e^{\Theta(d)}$.
% Moreover,  we have \begin{eqnarray}
% P_0(w,m) = \Phi(-\frac{w^\top \mu}{\|w\|_\Sigma}-m),\quad  P_1(w,m) = \Phi(\frac{w^\top \mu}{\|w\|_\Sigma}-m) 
% \end{eqnarray}
% where $\Phi$ is the Gaussian cumulative distribution function (CDF).  Thus, $P_0(w,m) \equiv P_1(-w,m)$ and the underlying classification problem is symmetric in the sense of Definition \ref{df:symmetric}.


\subsection{Training Data, Data Pruning, and Downstream Model}
Let $D_N=\{(x_1,y_1),\ldots,(x_N,y_N)\}$ be a dataset of $N$ iid pairs from the true distribution $P$ and let $D_N'=\{(x_1,y_1'),\ldots,(x_N,y_N')\}$ a version of the dataset (also iid) with labels $y'_i$ instead of $y_i$. For example, this could be labels generated by an AI trying to reproduce real-world data. $D'_N$ is the data on which the downstream model is trained.  

We will consider a family of models given by
\begin{eqnarray}
\mathbb P (y =1\mid x,w) = \hat y := \sigma(x^\top w) \in (0,1),
\end{eqnarray}
parametrized by a vector of weights $w \in \mathbb R^d$. Here, $\sigma$ is the sigmoid function defined by
\begin{eqnarray} 
\sigma(z):=\frac{1}{1+e^{-z}}.
\end{eqnarray}
For the loss function, we use binary cross-entropy (BCE), defined by
\begin{eqnarray}
    \ell(\hat y,y) = -y\log\hat y - (1-y)\log (1-\hat y).
\end{eqnarray}
Let $\widehat w_N$ be obtained via logistic regression fitted on $D'_N$ with ridge regularization parameter $\lambda>0$. Thus, $\hat w$ is the unique\footnote{Unicity is due to strong convexity of objective function.} minimizer of the following objective function
\begin{eqnarray}
L(w) := \frac{1}{N}\sum_{i=1}^N q_i\ell(\sigma(x_i^\top w), y_i') + \frac{\lambda}{2}\|w\|^2.
\label{eq:objective}
\end{eqnarray}
Here $q_i$ is a bit which indicates whether the $i$th training example has survived pruning. The numbers $q=(q_1,\ldots,q_N)$ is called a \emph{pruning strategy}. The corresponding downstream classifier is $\widehat f_N = f_{\widehat w_N}$, where the notation $f_w$ refers to the linear classifier induced by a weights vector $w \in \mathbb R^d$, i.e
\begin{eqnarray}
 f_w(x) := \begin{cases}
1,&\mbox{ if }x^\top w > 0,\\
0,&\mbox{ otherwise.}
\end{cases}
\end{eqnarray}
The test accuracy of the downstream model $\widehat f_N$ is defined by
\begin{eqnarray}
    acc(\widehat f_N) := \mathbb P(\widehat f_N(x) = y),\text{ for a random test point }(x,y) \sim P.
\end{eqnarray}
This quantity will be the main object of our analysis, and we will be interested in how it depends on the corruption level $p$ and the choice of pruning strategy $q$, in the infinite-sample limit $N \to \infty$.

For later reference, we also define an empirical version, namely the accuracy of $\widehat f_N$ evaluated on the clean dataset $D_N$, namely
\begin{eqnarray}
        \widehat{acc}(\widehat f_N) := \frac{1}{|M|}|\{i \in M \mid \widehat f_N(x_i) = y_i\}|,
\end{eqnarray}
where $M := \{i \in [N] \mid q_i = 1\}$ collects the indices of training samples which survive pruning by $q$.

\subsection{A Class of Parametrized Pruning Strategies}
Given hyper-parameters $\phi,\psi \in [0,1]$, we consider a broad class of parametrized pruning strategies with the following properties.
\begin{itemize}
    \item The weights $q_1,\ldots,q_N \in \{0,1\}$ are independent. Thus, whether any training example $(x_i,y_i')$ survives pruning or not is independent of what happens to the other examples. 
    \item The inclusion of an example does not depend on the specific labels attributed to this example by the ground-truth labeller $w_*$ or the fake labeller $w_{gen}$, it only depends on whether these labels coincide or not.
   % \item Conditioned on $y_i=k$ and $y'_i = \ell$, the distribution of $q_i$ is Bernoulli with parameter $\phi$ if $k = \ell$ and $\psi$ if $k \ne \ell$. Here, $\psi,\phi \in [0,1]$ are fixed parameters which completely characterize a pruning strategy $q$. % We shall usually write $(\phi,\psi)$ to mean the corresponding strategy $q$.
\end{itemize}
\begin{lemma}
\label{lm:margin-based}
    The above properties are verified when $P$ is a (balanced) Gaussian mixture, the fake data generator is linear model, i.e $y'_i = \operatorname{sign}(x_i^\top w_{gen})$ for some weights vector $w_{gen} \in \mathbb R$, and the pruning strategy is of the form
    \begin{eqnarray}
    q_i = 1[y_i(x_i^\top w_{prune})>0],
    \end{eqnarray}
    for some weights $w_{prune} \in \mathbb R^d$.
\end{lemma}



The above properties mean that, for any class labels $k,\ell \in \{0,1\}$, the random variables $(z_{ik\ell})_{i \in [N]}$ defined by $z_{ik\ell}=1[y_i=k,y_i'=\ell,q_i=1]$ are iid with Bernoulli distribution $Bern(p_{k\ell})$, where
\begin{eqnarray}
\label{eq:pkl}
    \begin{split}
p_{k\ell} &= \mathbb P(q_i = 1, y'_i=\ell,y_i=k)\\
&= \mathbb P(q_i=1 \mid y'_i=\ell,y_i=k)\mathbb P(y_i'=\ell \mid y_i=k)\mathbb P(y_i=k)\\
&=
\begin{cases}
    \phi_k(1-p)/2,&\mbox{ if }k=\ell,\\
    \psi_{k\ell}p/2,&\mbox{ else.}
\end{cases}    
    \end{split}
\end{eqnarray}
and the numbers $p$, $\phi_k$ and $\psi_{k\ell}$ are defined by
\begin{eqnarray}
p := \mathbb P(y'_i\ne y_i),\quad \phi_k = \mathbb P(q_i = 1 \mid y'_i=k,y_i=k),\quad \psi_{k\ell}= \mathbb P(q_i = 1 \mid y'_i=\ell,y_i=k).
\end{eqnarray}
Consequently, if $N_{k\ell}$ is the number of training examples that have true label $k$, fake label $\ell$, and survive pruning, then
\begin{eqnarray}
\label{eq:Nkl}
N_{k\ell} := \sum_{i=1}^N z_{ik\ell}
\end{eqnarray}
which is has binomial distribution $Bin(N,p_{k\ell})$. For simplicity of exposition, we shall focus on the case where
\begin{eqnarray}
    \phi_1 = \phi_0 = \phi,\quad \psi_{01}=\psi_{10} = \psi.
\end{eqnarray}
\begin{definition}
\label{df:rlhf-pruning}
Such a pruning strategy will be referred to as an RLHF-type strategy, where RLHF stands for Reinforcement Learning with Human Feedback.

It can be likened to the sense in which the term is classically used, where one assumes access to a strong oracle (e.g a human) who can tell apart bugguous predictions, but can also make mistakes.
\end{definition}
 \ElvisIssue{Link to FC's experiments. Beam-size should map to some value of $(\phi,\psi)$.} \julia{How? Please elaborate or erase.}
 \begin{remark}
    Note that the parametrization $(\phi,\psi)$ and $(p_{00},p_{11})$ describe the same RLHF-type policy via the following bijective transformation.
    \begin{align}
        p_{00} &= p_{11} = (1-p)\phi/2,\quad p_{01}=p_{10} = 
 p \psi /2.
    \end{align}
\end{remark}

\subsection{Examples}
Let us present some notable examples of pruning RLHF-type pruning strategies (Definition \ref{df:rlhf-pruning}).

\paragraph{No Pruning.} The case $(\phi,\psi) = (1,1)$ corresponds to no pruning, i.e the entire training dataset is used. %This is reminiscent of classical machine learning. \julia{hahaha. I like ``reminiscent". }
     \paragraph{Pure RLHF.} The case $(\phi,\psi) = (1,0)$. The pruning strategy only keeps indices corresponding to examples in the dataset which have correct label (all corrupted labels discarded). 

\paragraph{Margin-Based Pruning.} Let $w_{prune} \in \mathbb R^d$, and consider the pruning strategy defined by
    \begin{eqnarray}
    \label{eq:margin-based}
    q_i = 1[y_i(x_i^\top w_{prune})>0].
    \end{eqnarray}
    % where $z'_i := 2y_i'-1$. Note that $z'_ix_i^\top w$ is the margin of $(x_i,y_i')$ w.r.t to the decision boundary of the linear model $f_w(x) := \mathrm{sign}(x^\top w)$. In Lemma \ref{lm:margin-based}, we show that for symmetric classification problem (refer to Definition \ref{df:symmetric}), such a pruning scheme is in fact an instance of an RLHF-type pruning scheme with parameters $\phi=P_1(w,m)$ and $\psi=P_0(w,m)$, where the $P_k(w,m)$' are as defined in \eqref{eq:Pk}.
    This pruning strategy simplify filters out all examples on which it disagrees on the assigned label. 

\julia{Elivs, what to do with the below blue paragraph? Just leave it there? Do you want to tie it to something?}

\bbb{In some cases we can derive analytical expressions for $p_{k \ell}$. 
For the Gaussian mixture distribution $P$ with isotropic covariance, we have
$$
p_{00} = p_{11} = \mathbb P(x^\top w_p > 0,\, x^\top w_g > 0 \mid y=1)\mathbb P(y=1) = \mathbb P(z_p >-\mu^\top w_p,\,z_g >-\mu^\top w_g)/2,
$$
where $(x,y) \sim P$, so that the distribution of $x$ conditioned on $y=1$ is $N(\mu, \Sigma)$ with $\Sigma=I_d$; $z_g:=z^\top w_g$ and $z_p:=z^\top w_p$, for $z \sim N(0,\Sigma)$.
Now, assume WLOG that $\|w_g\|=\|w_p\|=1$, and observe that $(z_g,z_p)$ is bivariate normal with variance $\sigma^2=1$ and correlation coefficient $\rho=w_p^\top w_g$. The joint pdf is thus
$$
f(u,v) = \frac{1}{2\pi\Delta}e^{-\frac{1}{2\Delta^2}(u^2+v^2-2\rho u v)} = \frac{1}{\sqrt{2\pi\Delta^2}}e^{-\frac{1}{2\Delta^2}(v-\rho u)^2}\frac{1}{\sqrt{2\pi}}e^{-u^2/2},
$$
where $\Delta=\sqrt{1-\rho^2}$. We deduce that
\begin{align*}
   2 p_{00} &= \int_{-\mu^\top w_g}^\infty \left(\int_{-\mu^\top w_p}^\infty \frac{1}{\sqrt{2\pi\Delta^2}}e^{-\frac{1}{2\Delta^2}(v-\rho u)^2}\mathrm dv\right)\varphi(u)\mathrm du\\
    &= \int_{-\mu^\top w_g}^\infty\Phi\left(\frac{\rho u+\mu^\top w_p}{\Delta}\right)\varphi(u)\mathrm du\\
    &= \int_0^\infty \Phi\left(\frac{\rho (u + \mu^\top w_g) + \mu^\top w_p}{\Delta}\right)\varphi(u+\mu^\top w_g)\mathrm du.
\end{align*}
One can derive similar expressions for $p_{01}=p_{10}$,
namely
\begin{align*}
2p_{01} = \int_0^\infty \Phi\left(\frac{\rho (u - \mu^\top w_g) - \mu^\top w_p}{\Delta}\right)\varphi(u-\mu^\top w_g)\mathrm du.
\end{align*}
}

% The following theorem will be useful in the sequel
% \begin{theorem}
%     For the case of margin-based pruning, it holds that
%     \begin{align}
%     p &= \theta_{gen},\\
%         p_{00} &= p_{11} = \frac{1}{2} - \frac{1}{4\pi}(\theta_{gen} 
% + \theta_{prune} + \theta_{gp}),\\
% p_{01} &= p_{10}  = \frac{1}{4\pi}(\theta_{gen} + \theta_{p} - \theta_{gp}).
%     \end{align}
% where $\theta_{gen} \in [0,\pi]$ is the angle between $w_{gen}$ and $w_*$; $\theta_{prune} \in [0,\pi]$ is the angle between $w_{prune}$ and $w_*$; $\theta_{gp} \in [0,\pi]$ is the angle between $w_{gen}$ and $w_{prune}$.

% In particular, the following hold.

% (A) \textbf{Perfect Generator.} If $w_{gen}=w_*$, then
%     $p = 1/2,\, p_{00} = p_{11} = (1-\theta_{prune})/2,\, p_{01}=p_{10}=0$.
    
% (B) \textbf{Perfect Pruner.} If $w_{prune}=w_*$, then
% $p_{00} = p_{11}=(1-p)/2,\, p_{01}=p_{10}=0$.

% (C) \textbf{No Pruning.} If $w_{prune}=w_{gen}$
%     $p = 1/2,\, p_{00} = p_{11} = (1-p)/2,\, p_{01} = p/2$.
% \end{theorem} 
% \begin{proof}
%     $(x^\top w_{gen},x^\top w_{prune}, x^\top w_{prune})$ have a trivariate Gaussian distr;
% \end{proof}
% As we shall see, the downstream test accuracy (on clean data!) exhibits a sharp phase-transition across the manifold $p_{00}=p_{01}$, i.e $\theta_{gen}+\theta_{prune} = \pi$, or equivalently, $\theta_{prune} = (1-p)\pi$.
% \begin{mdframed}
% \textbf{Criticality.} The test accuracy is $100\%$ for $p < 
%  (1 - \epsilon)p_{crit}$ and $0\%$ for $p > (1 +\epsilon)p_{crit}$,
% where
% \begin{eqnarray}
% p_{crit} := 1-\theta_{prune}/\pi,
% \end{eqnarray}
% i.e test accuracy of the pruner (seen as a classifier).
% In particular, for the case of no-pruning (here corresponding to $w_{prune} = w_{gen})$, one has $\theta_{prune} = \theta_{gen} = 1-p$, and so $p_{crit} = 1/2$, which is not surprising. For smaller values of $\theta_{prune}$ (i.e $w_{prune}$ close to the ground-truth $w_*$), this breakpoint $p_{crit}$ becomes bigger, reflecting a higher tolerance to fake data.  \ElvisIssue{This perhaps provides an indirect explanation for some of the results of FC. Please check!}
% \end{mdframed}
 

% \subsection{A Generalization}
%   We can easily extend the definition of RLHF-type pruning strategies (Definition \ref{df:rlhf-pruning}) by considering a more general form for the $p_{k\ell}$'s appearing in \eqref{eq:pkl}, viz
%     \begin{eqnarray}
%         p_{k\ell} = \begin{cases}
%             (1-p)\phi_k/2,&\mbox{ if }k = \ell,\\
%             p\psi_{k\ell}/2,&\mbox{ if }k \ne \ell,
%         \end{cases}
%     \end{eqnarray}
%     for some scalars $\phi_0,\phi_1,\psi_{01},\psi_{10}\in [0,1]$. For simplicity of exposition, we only consider the special case above where $\phi_k=\phi$ and $\psi_{k\ell}=\psi$ for all $k,\ell$, giving \eqref{eq:pkl}. With this modification, every margin-based pruning strategy $(w,m)$ on a binary classification problem (symmetric or not, in the sense of Definition \ref{df:symmetric}) is a generalized RLHF-type pruning strategy with parameters
%     \begin{eqnarray}
%         \phi_{00} = P_0(-w,m),\quad \phi_{11}=P_1(w,m),\quad \psi_{01}=P_0(w,m),\quad \phi_{10}=P_1(-w,m),
%     \end{eqnarray}
%     where the $P_k(w,m)$'s are as defined in \eqref{eq:Pk}.

\subsection{Performance Bounds for Models Trained with RLHF Pruning}
    \begin{figure}[!htb]
    \centering
        \includegraphics[width=.45\textwidth]{RLHF.png}
        \includegraphics[width=.43\textwidth]{thresholds.png}
    % \includegraphics[width=.45\textwidth]
    % {prune.png}
   \caption{\textbf{Empirical Confirmation of Theorem \ref{thm:main}.} Comparing the breakdown points of different models. Here, the task is classifying a Gaussian mixture, with infinite training samples from datasets generated from a model with classification error rate $p$ (x-axis). Notice the sharp phrase-transitions where the model suddenly switches from perfect accuracy to worse-than-chance, a phenomenon predicted by Theorem \ref{thm:main}. % \textbf{Top Right.} "SD" stands for self-distillation, and "xn" means iterative self-distilling the same model $n$ times. Notice how a model pruning with a teacher's margin is already stronger than a few distillations (here it seems to actually matches double-distillation), and much stronger than the original student. Also notice how repeated self-distillation approaches RLHF. 
    \textbf{Left.} Performance of RLHF-type pruning strategies with different values of the  hyper-parameters $(\phi,\psi)$. Recall that the case $\psi/\phi=1$ corresponds to no pruning, while $\psi/\phi=0$ corresponds to pure RLHF. \textbf{Right.} Comparing $p_{up}$, approximated with $\sup\{p \mid acc(\widehat f_N) \ge 90\%\}$ (computed empirically), against the analytic estimate $p^-_\star(t)$ given in \ref{thm:main} (for $t=0.1$). Again, the results are in excellent agreement with the predictions of Theorem \ref{thm:main}. 
    % Even for $p > 1/2$, notice how the models with $\psi/\phi<1$ still continue to perhaps above chance level ($50\%$ accuracy). % \textbf{Bottom.} Comparing with margin-based pruning strategies. Again, notice the sharp phrase-transitions predicted by Theorem \ref{thm:main}.
    }
    \label{fig:curves}
\end{figure}
The following is one of our main results (proved in Appendix \ref{sec:proof}).
\begin{theorem}
\label{thm:main}
Suppose Condition \ref{cond:main} is in order. Fix $\phi,\psi,t \in (0,1)$ and define $p^\pm_\star(t) \in (0,1)$ by
\begin{eqnarray}
    p^-_\star(t) := \frac{1 - t}{1 - t + (1 + t)\psi/\phi},\quad p^+_\star:=\frac{1 + t}{1 + t + (1 - t)\psi/\phi}
    \label{eq:threshold}
\end{eqnarray}
If $p < p^-_\star(t)$, then the limit $N \to \infty$ it holds w.p $1-o(1)$  that the $acc(\widehat f_N) = 100\%$ for a downstream model $\widehat f_N$ trained on data from  a generator with error rate $p$ pruned with an RLHF-type strategy  with parameters $(\phi,\psi)$.

On the other hand, if $p > p^+_\star$, then the limit $N \to \infty$ it holds w.p $1-o(1)$  that the $acc(\widehat f_N) = 0\%$ for a downstream model $\widehat f_N$.

Thus, there is a sharp phase-transition around the corruption level $p_\star := 1/(1+\psi/\phi)$: as $p$ is increased past level $p_\star$, the downstream model $\widehat f_N$ abruptly switches from being perfectly accurate, to perfectly inaccurate!
\end{theorem}
See Figure \ref{fig:curves} for an empirical illustration of the theorem.

The thresholds $p^\pm_\star(t)$ appearing in the above theorem are proxies for the so-called \emph{breakdown points} $p_{up} \ge p_{down}$ defined by
\begin{align}
    p_{up} &= \inf\left\{p \in [0,1] \,\big|\, acc(\widehat f_N) \overset{a.s}\to 0\%\text{ in the limit }N \to \infty\right\},\\
        p_{down} &= \sup\left\{p \in [0,1] \,\big|\, acc(\widehat f_N) \overset{a.s}\to 100\%\text{ in the limit }N \to \infty\right\}.
\end{align}
Theorem \ref{thm:main} implies $p_{down} \ge p^-_\star(t)$ and $p_{up} \le p^+_\star(t)$ for all $t \in (0,1)$. Consequently,
\begin{corollary}
    Under the hypotheses of Theorem \ref{thm:main}, it holds that $p_{up} = p_{down}$.
\end{corollary}

\subsection{Some Consequences of Theorem \ref{thm:main}}
We now present some illustrious applications of Theorem \ref{thm:main}. These examples are empirically confirmed in Figure \ref{fig:curves}.


\paragraph{No Pruning.}
Here, we have $\psi/\phi=1$ and so the downstream model achieves $100\%$ accuracy for all values of corruption parameter $p$ up to the proxy  breakdown point predicted by Theorem \ref{thm:main} is then $p^-_\star = 1/2-t/2$.

\paragraph{Pure RLHF.} For this scenario, $\psi/\phi=0$ and  so Theorem \ref{thm:main} predicts that the downstream model $\widehat f_N$ achieves $100\%$ accuracy for all values of corruption parameter $p$ up to the breakdown point $p^-_\star = 1$. This is perhaps not so surprising in hindsight. The point is that even for moderately large values of $\psi/\phi$, the proxy breakdown point $p^-_\star$ given in \eqref{eq:threshold} can still be quite close to $1$.

\paragraph{Margin-Based Pruning.}
Consider Gaussian mixture data with means $\pm \mu$, and consider a margin-based pruning strategy in Lemma \ref{lm:margin-based}. It is clear that $\phi$ and $\psi$ only depend on all the 3 angles between the set of vectors $\{w_*,w_{gen},w_{prune}\}$, with $w_*=\mu$. \yunzhen{One might use a $w_{prune}$ with similar or better performance compared to $w_{gen}$; however, the selected data may not show improvement beyond $w_{gen}$. This explains why using LLaMA3 does not enhance selection.}

\subsection{Sketch of Proof of Theorem \ref{thm:main}}
The proof is based on the following representation (refer to Proposition \ref{prop:acc}) of the accuracy of the downstream classifier $\widehat f_N$ evaluated on the the clean training dataset $D_N$, namely
\begin{eqnarray}
\widehat{acc}(\widehat f_N) = \frac{N_{11}1_{\overline A < 1/2} + N_{00} 1_{\overline D < 1/2} + N_{10}1_{\overline B > 1/2} + N_{01} 1_{\overline C > 1/2}}{N_{11} + N_{00} + N_{10} + N_{01}},
\end{eqnarray}
for some random some random variables $\overline A,\overline B,\overline C,\overline D \in (0,1)$ which depend on the $N_{k\ell}$'s defined in \eqref{eq:Nkl}. By classical results in learning theory (e.g., see \cite{kakade2008complexity}), we know that the gap to the population version (test accuracy) $acc(\widehat f_N)$ shrinks to zero at rate $O(1/N)$, and so since the claim in Theorem \ref{thm:main} is made only in the limit $N \to \infty$, we are good.  

Next, in Proposition \ref{prop:symmetric-case} and Proposition  \ref{prop:skewed-case}, necessary and sufficient conditions are established to ensure $\overline A,\overline D < 1/2$ and $\overline B,\overline C > 1/2$, and therefore $\widehat{acc}(\widehat f_N) = 100\%$. These conditions are given explicitly in terms of the $N_{k\ell}$'s. Finally, in Proposition \ref{prop:concentration}, concentration of measure is used to control the $N_{k\ell}$'s, and present the aforementioned conditions in terms of the $p_{k\ell}$'s defined in \eqref{eq:pkl}, and therefore in terms of $p$, $\phi$, and $\psi$ alone, giving condition \eqref{eq:threshold}.
\label{prop:acc-informal}


==> proofs.tex <==
\input{theory.tex}

\section{Proof of Theorem \ref{thm:noisyhutter}}
We will need the following lemma (proved later).
\begin{lemma}
\label{lm:Borell-TIS}
    For any $x$, it holds that $\hat f_T(x) = f_0(x)$ except on an event $\mathcal E_T(x)$ which has probability at most $e^{-C' p(x)T}$ for some constant $C'>0$ which only depends on $\pi$.
\end{lemma}
\paragraph{Upper-Bound.}
Thanks to Lemma \ref{lm:Borell-TIS}, we have
\begin{equation*}
\begin{split}
    \err(\hat f_T) &= \mathbb P_{x,y,D_T}(\hat f_T(x) \ne y)\\
    &= \sum_{x,y}p(x,y)\left(\mathbb P_{D_T}(\hat f_T(x) \ne y \mid \mathcal E_T(x))\mathbb P(\mathcal E_T(x))+\mathbb P_{D_T}(\hat f_T(x) \ne y \mid \mathcal E_T(x)^c)\mathbb P(\mathcal E_T(x)^c)\right)\\
    &= \sum_{x,y}p(x,y)\left(\mathbb P_{D_T}(\hat f_T(x) \ne y \mid \mathcal E_T(x))\mathbb P(\mathcal E_T(x))+1_{y \ne f_0(x)}\mathbb P(\mathcal E_T(x)^c)\right).
\end{split}
\end{equation*}
Now, one computes
\begin{eqnarray*}
\begin{split}
   \sum_{x,y}p(x,y) 1_{y \ne f_0(x)}\mathbb P(\mathcal E_T(x)^c) &= \sum_x p(x)\mathbb P(y \ne f_0(x)) \mathbb P(\mathcal E_T(x)^c)\\
   &= (1-\pi-\frac{1-\pi}{M})\sum_x p(x)(1-\mathbb P(\mathcal E_T(x))\\
   &= \err_\star((1-\sum_x p(x)\mathbb P(\mathcal E_T(x))))\\
   &= \err_\star + O\left(\sum_x p(x)\mathbb P(\mathcal E_T(x))\right).
\end{split}
\end{eqnarray*}
On the other hand
\begin{eqnarray*}
    \begin{split}
\sum_{x,y}p(x,y)\mathbb P_{D_T}(\hat f_T(x) \ne y \mid \mathcal E_T(x))\mathbb P(\mathcal E_T(x)) &\le \sum_{x,y}p(x,y)\mathbb P(\mathcal E_T(x)) =\sum_x p(x)\mathbb P(\mathcal E_T(x)).
    \end{split}
\end{eqnarray*}
Thus, $0 \le \err(\hat f_T) - \err_* \lesssim \sum_x p(x) P(\mathcal E_T(x))$. Observing that
$$
\sum_x p(x) P(\mathcal E_T(x)) \le \sum_x p(x) e^{-C'Tp(x)\pi} \lesssim (C' T)^{-c} \lesssim T^{-c},
$$
the upper-bound follows.

\paragraph{Lower-Bound.}

$n_T(x,y) = $
\qed

\section{Technical Proofs}
\subsection{Proof of Theorem \ref{thm:bessel}}
Indeed, one computes
\begin{equation*}
    \begin{split}
        acc(w) := \mathbb P_{(x,y) \sim P}(yf_w(x) \ge 0) = 2\mathbb E_{x \sim N(0,I_d)}[H(x^\top w_*)H(x^\top w)] = \ldots = 1-\theta/\pi.
    \end{split}
\end{equation*}
where $H$ is the Heaviside function. \qed

\subsection{Proof of Lemma \ref{lm:Borell-TIS}}
\paragraph{The Noise Term.} For any $x \in \mathbb N_*$ and $y \in [M]$, the random variable $n_T(x,y)$ has mean $p(x,y) T = p(x)\left((1-\pi)/M + \pi \delta_{f_0(x)}(y)\right)T$. For any other $y' \in [M]$, one computes
\begin{eqnarray*}
\begin{split}
&\mathbb E\, n_T(x,y)n_T(x,y') =  \sum_{s,t} \mathbb E\, [Z_s(x,y) Z_t(x,y')] = \sum_{s,t}\mathbb P((x_s,y_s) = (x,y),\,(x_t,y_t) = (x,y'))\\
&= \delta_{y=y'}\cdot \sum_s \mathbb P((x_s,y_s) = (x,y)) + \sum_s \mathbb P((x_s,y_s) = (x,y))\cdot \sum_{t \ne s}\mathbb P((x_t,y_t) = (x,y'))\\
&= \delta_{y=y'}\cdot p(x,y)T + p(x,y)p(x,y')T(T-1).
\end{split}
\end{eqnarray*}

Thus, the covariance $C_{yy'}(x)$ of $n_T(x,y)$ and $n_T(x,y')$ is given by
\begin{eqnarray*}
\begin{split}
C_{yy'}(x) &= \mathbb E\, n_T(x,y)n_T(x,y') - \mathbb E\, n_T(x,y)\mathbb E\,n_T(x,y')\\
&= p(x,y)\delta_{y=y'} T + p(x,y)p(x,y')T(T-1) - p(x,y)p(x,y')T^2\\
&= \begin{cases}
p(x,y)T+p(x,y)^2 T(T-1)-p(x,y)^2T^2=p(x,y)(1-p(x,y))T,&\mbox{ if }y=y',\\
p(x,y)p(x,y')T(T-1)-p(x,y)p(x,y')T^2 = -p(x,y)p(x,y')T,&\mbox{ if }y \ne y'
\end{cases}
\\
&= p(x,y)(\delta_{y=y'}-p(x,y'))T
\end{split}
\end{eqnarray*}
% We conclude that $C(x) = (I_M - u_x u_x^\top)T \in \mathbb R^{M \times M}$ where $u_x$ is the $M$-dimensional vector with coordinates given by $u_x(y) := p(x,y)$.
Observe that for any distinct $y,y' \in [M]$, one has
\begin{eqnarray*}
\begin{split}
\mathbb E\, (n_T(x,y) - n_T(x,y'))^2 &= p(x,y)(1-p(x,y)) T + p(x,y')(1-p(x,y'))T - 2p(x,y)p(x,y')T\\
&\le p(x,y)T-p(x,y')T - 2p(x,y)p(x,y')T = (p(x,y)-p(x,y'))^2 T.
\end{split}
\end{eqnarray*}
\begin{mdframed}
Let us pretend that the $n_T(x,y)$'s are Gaussians with covariance structure given by the $C_{yy'}(x)'s$. Since we'll be interested in the limit $T \to \infty$, this approximation is justified by the CLT!
\end{mdframed}
We deduce from the Sudakov-Fernique inequality that
$$
\mathbb E\, \max_{y \ne f_0(x)} n_T(x,y) \le p(x)\frac{1-\pi}{M} T + (C/2)\max_{y \ne f_0(x)} p(x,y)T\log M \le C p(x)T\cdot (1-\pi)\frac{\log M}{M},
$$
for some absolute constant $C>0$.
Now, define
$$
\sigma^2 := \max_{y \ne f_0(x)} C_{yy}(x) = \max_{y \ne f_0(x)} p(x,y)(1-p(x,y))T = a(x)(1-a(x)) T,
$$
with $a(x) := p(x)(1-\pi)/M$. The Borell-TIS inequality tells us that for any $\lambda > 0$,
\begin{eqnarray*}
    \begin{split}
\mathbb P\left(\max_{y \ne f_0(x)} n_T(x,y) \ge Cp(x)(1-\pi)\frac{\log M}{M} + \lambda \right) &\le \mathbb P\left(\max_{y \ne f_0(x)} n_T(x,y) \ge \mathbb E\, \max_{y \ne f_0(x)} n_T(x,y)+ \lambda \right)\\
&\le e^{-\lambda ^2/(2\sigma^2)}.
    \end{split}
\end{eqnarray*}
Taking $\lambda = p(x)T \cdot (1-\pi)\log(M)/M$ gives
\begin{eqnarray}
\max_{y \ne f_0(x)} n_T(x,y) \le C p(x)T\cdot (1-\pi)\frac{\log M}{M}\text{ w.p }1-e^{-p(x)T}. 
\label{eq:noiseterm}
\end{eqnarray}

\paragraph{The Signal Term.} 
On the other hand, binomial concentration gives
$$
n_T(x, f_0(x)) \ge \pi/2+(1-\pi)/M \ge \pi/2\text{ w.p }1-e^{-C' p(x) T},
$$

where $C' := \pi^3/12 >0$ only depends on $\pi$. Combining with \eqref{eq:noiseterm}, we deduce that: if
$$
\pi > \dfrac{C \log(M)/ M}{1/2+C\log(M)/M},
$$
then it holds w.p $1-2e^{-C'p(x) T}$ that $n_T(x,f_0(x)) > \max_{y \ne f_0(x)} n_T(x,y)$, i.e $\hat f_T(x) = f_0(x)$, as claimed. \qed



==> theory.tex <==

\section{Proof of Theorem \ref{thm:rlhf} (RLHF on Dirty Data Only)}
The proof will be very much inspired by the proof of Theorem 4.3 of Das and Sanghavi (2023) \url{https://openreview.net/forum?id=UL9purXHyB}.
\subsection{Preliminaries}
The dirty dataset $D'$ can always be realizable as follows. Let $n=N/2$ and $\overline n := |I_{bad}|/2$, assumed to be integers WLOG. The sets $I_{bad}$ and $I_{good}$ are as defined in \eqref{eq:pipes}.
\begin{itemize}
\item \textbf{Step 1.} Sample an $n$ data points iid from $P_{x|y=1}$, and independently of this, sample $n$ data points iid from $P_{x|y=0}$. 
\item \textbf{Step 2.} Form a vector of clean labels $Y  \in \{0,1\}^{2n}$ by setting
\begin{eqnarray}
y_i = \begin{cases}
    1,&\mbox{ if }1 \le i \le n,\\
    0,&\mbox{ if }n + 1 \le i \le 2n.
\end{cases}
\end{eqnarray}
\item \textbf{Step 3.} Collect all this $(x_i,y_i)$ pairs into a clean dataset $D$ of size $2n$.
\item \textbf{Step 4.} Form a vector of dirty labels $\overline Y=(\overline y_1,\ldots,\overline y_{2n}) \in \{0,1\}^{2n}$ by setting
\begin{eqnarray}
\begin{split}                                                
\overline y_i &= \begin{cases}
1-y_i,&\mbox{ if }i \in I_{bad},\\
y_i,&\mbox{ if }i \in I_{good}
\end{cases}\\
&= \begin{cases}
1-y_i = 0,&\mbox{ if }1 \le i \le \overline n,\\
y_i = 1,&\mbox{ if }\overline n + 1 \le i \le n,\\
1-y_i=1,&\mbox{ if }n+1 \le i \le n + \overline n,\\
y_i = 0,&\mbox{ if }n+\overline n + 1 \le i \le 2n,
\end{cases}
\end{split}
\end{eqnarray}
\item \textbf{Step 5.} Collect all this $(x_i,\overline y_i)$ pairs into a clean dataset $D'$ of size $2n$.
\end{itemize}
Note that  the sets $I_{bad}$ and $I_{good}$ defined in \eqref{eq:pipes} are now given by
\begin{align}
I_{bad} &:= \{1,\ldots,\overline n\} \cup \{n+1,\ldots,n+\overline n\},\\
I_{good} &= \{\overline n + 1,\ldots, n\} \cup \{n+\overline n + 1,\ldots,2n\}.
\end{align}
Define integers $n_1,n_2,n_3,n_4 \ge 0$ by 
\begin{align}
n_1: &= \sum_{j=1}^{\overline n} q_j,\quad n_2 := \sum_{j=\overline n + 1}^n q_j,\quad n_3 := \sum_{j=n+1}^{n+\overline n}q_j,\quad n_4 := \sum_{j=n+\overline n + 1}^{2n}q_j,
\end{align}
and observe that the integers $N_{keep}$, $N_{nice}$, and $N_{nasty}$ defined in \eqref{eq:pipes} can be rewritten as 
\begin{eqnarray}
N_{keep} := n_1+n_2+n_3+n_4,\quad N_{nice} = n_2+n_4,\quad N_{nasty} := N_{keep}-N_{nice} = n_1+n_3.
\end{eqnarray}


\subsection{Key Derivations}
Let us start by observing that
\begin{eqnarray}
\begin{split}
\partial_{\hat y}\ell(y,\hat y) &= -\frac{y}{\hat y} + \frac{1-y}{1-\hat y} = -\frac{y-\hat y}{\hat y(1-\hat y)},\\
\sigma'(v) &= \frac{e^{-v}}{(1+e^{-v})^2} = \sigma(v)(1-\sigma(v)) = \hat y(1-\hat y).
\end{split}
\end{eqnarray}
Using the chain rule, we deduce that the following well-known identity
$$
\nabla_\theta \ell(\hat y,y) = \sigma'(v)\partial_{\hat y}\ell(y,\hat y)\nabla_\theta(x^\top \theta) = (\hat y - y)x.
$$
One then computes the gradient of $L$ as follows
\begin{eqnarray}
\begin{split}
\nabla L(\theta) &= \sum_{i=1}^{2n} (\hat y_i - \overline y_i)q_i x_i + \gamma \theta = -\left(\sum_i q_i\alpha_i x_i - \theta\right)\gamma,\\
\text{ with }
\alpha_i &:= \frac{\overline y_i-\sigma(v_i)}{\gamma},\quad v_i := x_i^\top \theta.
\end{split}
\end{eqnarray}
The KKT conditions $\nabla L(\theta)=0$ translate to
\begin{eqnarray}
\theta = \sum_{i=1}^{2n} q_i\alpha_i x_i.
\end{eqnarray}
Now, thanks to the structural assumptions, for any $i \in [2n]$, one has
\begin{eqnarray}
\begin{split}
v_i &= x_i^\top \theta = \sum_{j=1}^{2n} \langle x_i, x_j\rangle\alpha_j = \sum_{j=1}^{n} \langle x_i, x_j\rangle\alpha_j + \sum_{j=n + 1}^{2n} \langle x_i, x_j\rangle\alpha_j\\
&= q_i\alpha_i + \begin{cases}
a\left(\sum_{j=1}^nq_j\alpha_j-q_i\alpha_i\right) + b\sum_{j=n+1}^{2n}q_j\alpha_j,&\mbox{ if }1 \le i \le n,\\
b\sum_{j=1}^nq_j\alpha_j + a\left(\sum_{j=n+1}^{2n}q_j\alpha_j-q_i\alpha_i\right),&\mbox{ if }n + 1 \le i \le 2n
\end{cases}\\
&= \begin{cases}
\delta q_i\alpha_i+as+bt,&\mbox{ if }1 \le i \le n,\\
\delta q_i\alpha_i + at + bs,&\mbox{ if }n+1 \le i \le 2n,
\end{cases}
\end{split}
\end{eqnarray}
where $s := \sum_{j=1}^n q_j\alpha_j$, $t := \sum_{j=n+1}^{2n}q_j\alpha_j$, and we have used the definition $\delta:=1-a$. This yields
\begin{eqnarray}
\begin{split}
\gamma \alpha_i &= \overline y_i-\sigma(v_i) = \begin{cases}
-\sigma(\delta q_i\alpha_i + as + b t),&\mbox{ if }1 \le i \le \overline n,\\
1-\sigma(\delta q_i\alpha_i + as + b t),&\mbox{ if }\overline n + 1\le i \le n,\\
1-\sigma(\delta q_i\alpha_i + at + bs),&\mbox{ if }n+1 \le i \le n + \overline n,\\
-\sigma(\delta q_i\alpha_i + at + bs),&\mbox{ if }n+\overline n + 1 \le i \le 2n.
\end{cases}
\end{split}
\end{eqnarray}
Due to monotoneicity of the sigmoid function $\sigma$, we deduce that: there exist scalars $\alpha,\overline \alpha,\beta,\overline \beta \ge 0$ such that for any $i \in \mathrm{supp}(q)$, it holds that
\begin{eqnarray}
\alpha_i = \begin{cases}
-\overline \alpha,&\mbox{ if }1 \le i \le \overline n,\\
\alpha,&\mbox{ if }\overline n + 1 \le i \le n,\\
\overline\beta,&\mbox{ if }n + 1 \le i \le n + \overline n,\\
-\beta,&\mbox{ if }n+\overline n + 1 \le i \le 2n.
\end{cases}
\end{eqnarray}
Like in Das and Sanghavi (2023), it can be shown that
$$
\alpha=\beta,\quad \overline\alpha=\overline\beta.
$$
Now, one computes
\begin{align}
\alpha_i &= \begin{cases}
-\overline \alpha,&\mbox{ if }1 \le i \le \overline n,\\
\alpha,&\mbox{ if }\overline n + 1 \le i \le n,\\
\overline\alpha,&\mbox{ if }n + 1 \le i \le n + \overline n,\\
-\alpha,&\mbox{ if }n+\overline n + 1 \le i \le 2n.
\end{cases}\\
s &= \sum_{j=1}^n q_j\alpha_j= \sum_{j=1}^{\overline n}q_j\alpha_j + \sum_{j=\overline n + 1}^nq_j\alpha_j = -n_1\,\overline\alpha + n_2\alpha,\\%=n_q\alpha-\overline n_q(\alpha+\overline\alpha),\\
t &:= \sum_{j=n+1}^{2n}q_j \alpha_j = \sum_{i=n+1}^{n + \overline n}q_j\alpha_j + \sum_{j=n+\overline n + 1}^{2n}q_j\alpha_j = n_3\overline\alpha - n_4\alpha,\\%\overline n_q\,\overline\alpha -(n_q-\overline n_q)\alpha = -s,\\
v_i &= \begin{cases}
\delta \alpha_i+as+bt,&\mbox{ if }1 \le i \le n,\\
\delta \alpha_i + at + bs,&\mbox{ if }n+1 \le i \le 2n,
\end{cases}\nonumber\\
&= \begin{cases}
-\delta \overline \alpha+as+bt,&\mbox{ if }1 \le i \le \overline n,\\
\delta \alpha + as + bt,&\mbox{ if }\overline n+1 \le i \le n,\\
\delta \overline\alpha +at + bs,&\mbox{ if }n+1 \le i \le n+\overline n,\\
-\delta \alpha + at + bs,&\mbox{ if }n+\overline n + 1 \le i \le 2n,
\end{cases}\\
\gamma\alpha_i &= \overline y_i - \sigma(v_i) = \begin{cases}
-\sigma(-\delta \overline \alpha + as + bt),&\mbox{ if }1 \le i \le \overline n,\\
1-\sigma(\delta \alpha + as + bt),&\mbox{ if }\overline n+1 \le i \le n,\\
1-\sigma(\delta \overline\alpha + at + bs),&\mbox{ if }n+1 \le i \le n+\overline n,\\
-\sigma(-\delta \alpha + at + bs),&\mbox{ if }n+\overline n + 1 \le i \le 2n,
\end{cases}
\end{align}
Furthermore, we deduce that $\alpha,\overline \alpha$ must solve the the system of equations
\begin{mdframed}
    \begin{eqnarray}
\begin{split}
\gamma \overline \alpha &= \sigma(as+bt-\delta  \overline \alpha),\\
1-\gamma \alpha &= \sigma(as+bt + \delta \alpha),\\
\text{ with }s &= n_2\alpha - n_1 \overline \alpha,\quad t = n_3\overline\alpha - n_4\alpha.
\end{split}
\label{eq:implicit}
\end{eqnarray}
%\ElvisIssue{TODO: Use Maclaurin expansion of $\sigma$, namely $\sigma(z) = 1/2+z/4+O(z^2)$, to help solve the equations at least in some relevant regimes.}
\end{mdframed}
Note that in the above equations we must have
\begin{align}
0 < \alpha,\overline\alpha &< \frac{1}{\gamma}\label{eq:axiom1},\\
\alpha + \overline\alpha &< \frac{1}{\gamma}.
\label{eq:axiom2}
\end{align}
The first line is  because range of $\sigma$ is contained in $(0,1)$, and the second line is because
$$
\gamma \overline \alpha = \sigma(as+bt - \delta\overline \alpha) < \sigma(as+bt + \delta \alpha) = 1-\gamma\alpha.
$$
Consequently, the labels predicted by this model for any $i \in \mathrm{supp}(q)$ are given by
\begin{eqnarray}
\widehat y_i = \overline y_i-\gamma \alpha_i = \begin{cases}
\gamma \overline \alpha,&\mbox{ if }1 \le i \le \overline n,\\
1-\gamma \alpha,&\mbox{ if }\overline n + 1 \le i \le n,\\
1-\gamma\overline\alpha,&\mbox{ if }n + 1 \le i \le n + \overline n,\\
\gamma\alpha,&\mbox{ if }n+\overline n + 1 \le i \le 2n.
\end{cases}
\end{eqnarray}
Thus, the model's accuracy when evaluated on the clean training data is given by
\begin{eqnarray}
\begin{split}
    acc_{train} &= \frac{n_1+n_3}{2n}1_{\gamma\overline \alpha > \frac{1}{2}} + \frac{n_2+n_4}{2n}1_{\gamma \alpha \le \frac{1}{2}} + \frac{2n-N_{keep}}{2n}\\
    &= 1 - \frac{N_{nasty}}{2n}1_{\overline \alpha \le \frac{1}{2\gamma}} - \frac{N_{nice}}{2n}1_{\alpha > \frac{1}{2\gamma}}\\
    &= 1- \frac{N_{nice}}{2n}1_{\alpha > \frac{1}{2\gamma}}-\frac{N_{nasty}}{2n}1_{\overline \alpha \le \frac{1}{2\gamma}},
\end{split}
\end{eqnarray}
We deduce the following result.
\ElvisIssue{See "Pruning Theory" manuscript for correct definition of $acc_{train}$ which takes into account the selected mask. That is, we only consider the empirical average on the mask, not on the entire training set. This restricted average still converges to population version under mild conditions.}
\begin{proposition}
\label{prop:batman}
The condition
\begin{align}
\label{eq:key}
 \alpha \le \frac{1}{2\gamma} < \overline\alpha
\end{align}
is sufficient to ensure $100\%$ accuracy when the model is evaluated on the clean training dataset!
\end{proposition}

\subsection{Solving The System of Equations \eqref{eq:implicit}}
It is well-known that
\begin{eqnarray}
\sigma(z) = \frac{1}{2} + \frac{z}{4} + \epsilon(z),    
\end{eqnarray}
where the error function $\epsilon$ has the following properties which shall be crucial later:
\begin{itemize}
    \item The sign of $\epsilon$ is given by
$$
\begin{cases}
\epsilon(z) < 0,&\mbox{ for }z > 0,\text{ i.e for }\sigma(z) < 1/2,\\
\epsilon(z) = 0,&\mbox{ for }z = 0,\text{ i.e for }\sigma(z) = 1/2,\\
\epsilon(z) > 0,&\mbox{ for }z < 0,\text{ i.e for }\sigma(z) > 1/2.
\end{cases}
$$
\item $\epsilon$ is decreasing. In particular, this mean
\begin{align}
\sup_{z \,\mid\, \sigma(z) \in [\sigma(-1),1/2]}\epsilon(z) &= \sup_{z \in [-1,0]}\epsilon(z) = \epsilon(-1)<0.02,\\
\inf_{z \,\mid\, \sigma(z) \in [1/2,\sigma(1)]}\epsilon(z) &= \sup_{z \in [0,1]}\epsilon(z) = \epsilon(1)>-0.02.
\end{align}
\end{itemize}
For simplicity of exposition, henceforth assume $b=-a$, with $a \in (0,1)$ and recall the definition $\delta := 1-a \in (0,1)$. 

One can prove the following lemma directly from inspecting \eqref{eq:implicit}.
\begin{lemma}
  In the limit \eqref{eq:asymptotic}, the system of equations \eqref{eq:implicit} is solved by $(\alpha,\overline\alpha)$ given by
\begin{align}
         \alpha &= \frac{(1+\zeta)(1-\phi)}{\gamma + \delta/4},\quad \overline \alpha = \frac{(1+\zeta)\phi}{\gamma+\delta/4},
         \label{eq:alphas}
  \end{align}
  where $\zeta := \zeta_1 + \zeta_2$ is defined implicitly by
\begin{eqnarray}
    \zeta_1 := \epsilon(\sigma^{-1}(\gamma\overline\alpha)),\quad \epsilon(\sigma^{-1}(\gamma\alpha)).
\end{eqnarray}
  \end{lemma}
We will prove that $0 < \zeta \le 2\epsilon(-1) < 0.04$ under appropriate conditions on $\gamma$ in terms of $\phi$ and $\delta$.

Now, $v=\sigma^{-1}(s)$ implies $s=1/(1+e^{-v})$ and so $1+e^{-v} = 1/s$, i.e
$$
\sigma^{-1}(s) = -\log(1/s-1).
$$

By way of contradiction, suppose on the contrary that $\zeta < 0$. Then,
\begin{eqnarray}
\begin{split}
\gamma \overline \alpha &< \frac{\gamma \phi}{\gamma + \delta/4} \le \frac{1}{2},\\
\gamma \alpha &< \frac{\gamma(1-\phi)}{\gamma + \delta/4} \le \frac{\gamma \phi}{\gamma + \delta/4} \le \frac{1}{2},
\end{split}
\end{eqnarray}
provided we impose
$$
\phi \le \frac{\gamma+\delta/4}{2\gamma}.
$$

But then for $s \in \{\gamma\overline\alpha,\gamma\alpha\}$, it holds that $s < 1/2$, i.e $1/s-1 > 1$ and so $\sigma^{-1}(s) = -\log(1/s-1)<0$. We deduce that
$$
\zeta_1 = \epsilon(\sigma^{-1}(\gamma\overline\alpha)) > 0,\quad \zeta_2 = \epsilon(\sigma^{-1}(\gamma\alpha)) > 0.
$$
That is, $\zeta = \zeta_1 + \zeta_2 > 0$ which contradicts $\zeta<0$. Thus, we must have $\zeta > 0$. In particular, this implies
$$
\overline\alpha > \alpha.
$$

Next we prove that $\zeta \le 2\epsilon(-1) < 0.04$.  Now, under the condition
\begin{eqnarray}
\frac{\gamma(1-\phi)}{\gamma + \delta/4} \ge \sigma(-1) = \frac{1}{1+e},
\label{eq:wtf}
\end{eqnarray}
we must have $\gamma\overline \alpha, \gamma\alpha \ge \sigma(-1)$, in which case
$$
\zeta_1 := \epsilon(\sigma^{-1}(\gamma\overline\alpha)) \le \epsilon(-1) < 0.02,\quad \zeta_2 := \epsilon(\sigma^{-1}(\gamma\alpha)) \le \epsilon(-1),
$$
and so $\zeta := \zeta_1 + \zeta_2 \le 2\epsilon(-1)<0.04$. 

Observe that the condition \eqref{eq:wtf} is met if we impose
\begin{eqnarray}
    \label{eq:sweet1}
\phi \le 1-\frac{\gamma + \delta/4}{(1+e)\gamma}.
\end{eqnarray}
Finally, observe that: ensure $\alpha \le 1/2 < \gamma\overline\alpha$, it suffices to impose
\begin{eqnarray}
    \frac{1.04\gamma(1-\phi)}{\gamma + \delta/4} < \frac{1}{2} < \frac{\gamma\phi}{\gamma+\delta/4},\text{ i.e } \phi > \max\left(\frac{\gamma+\delta/4}{2\gamma},  1-\frac{\gamma + \delta/4}{2.08\gamma}\right).
    \label{eq:sweet2}
\end{eqnarray}

\subsection{Proof of Theorem \ref{thm:rlhf}}
  Thus, provided \eqref{eq:sweet1} and \eqref{eq:sweet2} are satisfied, $\alpha$ and $\overline\alpha$ are given as in \eqref{eq:alphas} with $\zeta \in (0,0.04)$ verify \ref{eq:key}. It follows from Proposition \ref{prop:batman} that accuracy on clean training dataset tends to $100\%$. Because of the condition $d=O(N)$, it then follows from uniform-convergence\footnote{Note that $d$ is the VC dimension of linear models} (VC theory) that the test accuracy of the model tends to $100\%$. This completes the proof of the theorem. \qed



==> theory_new.tex <==
\subsection{Data Distribution} 
Consider a probability distribution $P$ over $\mathbb R^d \times \{0,1\}$ with the following high-dimensional property
\begin{mdframed}
\begin{condition}
\label{cond:main}
Given $N \le N(d)$ iid samples $(x_1,y_1),\ldots,(x_N,y_N)$ from $P$ with $N \le N(d)$, the following hold estimates w.p $1-o(1)$ uniformly on all $i,j \in [N]$, in the limit $d \to \infty$
\begin{align}
    \|x_i\|^2 &\simeq 1\label{eq:unit-norm},\\
    x_i^\top x_j &\simeq \begin{cases}
        a,&\mbox{ if }y_i = y_j,\\
    b,&\mbox{ if }y_i \ne y_j\label{eq:cross-class-cor},
    \end{cases}
\end{align}
where $b < a < 1$ are constants. For simplicity of presentation of our results, We will further assume that $b=-a$ or $b=0$.
\end{condition}
\end{mdframed}
The above structural condition is inspired by an assumption in \cite{das2023understanding}.

\yunzhen{Can we move this condition to appendix? Or we state that our analysis works for this general case. Then we focus on a specific case on Gaussian mixtures and linear models.}

% and proposed a self-distillation as a way to boost accuracy for certain values of the corruption parameter $p$.
For simplicity of exposition, we will only consider balanced distributions, meaning that
\begin{eqnarray}
\mathbb P(y=1) = \mathbb P(y=0) = 1/2,\text{ for }(x,y) \sim P.
\end{eqnarray}
% \begin{definition}
% \label{df:symmetric}
%     For any $w \in \mathbb R^d$, $m \in \mathbb R$, and $k \in \{0,1\}$, define  $P_k(w,m) \in [0,1]$ by
%     \begin{eqnarray}
%         P_k(w,m) := \mathbb P(x^\top w > m \mid y=k),\text{ where }(x,y) \sim P.
%         \label{eq:Pk}
%     \end{eqnarray}
%     This is the probability that a random test point $x \in \mathbb R^d$ sampled from class label $k$ lies in the half-space $x^\top w - m > 0$. 
    
%     If $P_0(w,m) \equiv P_1(-w,m)$, we say the underlying classification problem is symmetric.
% \end{definition}

\paragraph{Gaussian Mixture Example.}
As a first example, in the case of Gaussian mixtures where the features have conditional distribution given by
\begin{eqnarray}
x \mid y \sim N(\mu_y,\Sigma),\\
\end{eqnarray}
where $\mu_y = (2y-1)\mu$, for some $\mu \in \mathbb R^d$ and positive-definite matrix $\Sigma$ with $\mathbb E\,\|x\|^2 = \|\mu\|^2+\operatorname{tr}\Sigma = 1$, we may take
\begin{eqnarray}
a=\|\mu\|^2,\quad b= -a. 
\end{eqnarray}
Condition \ref{cond:main} then holds thanks to concentration, with $N(d) = e^{\Theta(d)}$.
% Moreover,  we have \begin{eqnarray}
% P_0(w,m) = \Phi(-\frac{w^\top \mu}{\|w\|_\Sigma}-m),\quad  P_1(w,m) = \Phi(\frac{w^\top \mu}{\|w\|_\Sigma}-m) 
% \end{eqnarray}
% where $\Phi$ is the Gaussian cumulative distribution function (CDF).  Thus, $P_0(w,m) \equiv P_1(-w,m)$ and the underlying classification problem is symmetric in the sense of Definition \ref{df:symmetric}.


\subsection{Training Data, Data Pruning, and Downstream Model}
Let $D_N=\{(x_1,y_1),\ldots,(x_N,y_N)\}$ be a dataset of $N$ iid pairs from the true distribution $P$ and let $D_N'=\{(x_1,y_1'),\ldots,(x_N',y_N')\}$ a version of the dataset (also iid) with labels $y'_i$ instead of $y_i$. For example, this could be labels generated by an AI trying to reproduce real-world data. $D'_N$ is the data on which the downstream model is trained.  \yunzhen{I would like to have the linear model generate synthesized data with sigmoid function as simulation shows great difference between using sigmoid or not.}

We will consider a family of models given by
\begin{eqnarray}
\mathbb P (y =1\mid x,w) = \hat y := \sigma(x^\top w) \in (0,1),
\end{eqnarray}
parametrized by a vector of weights $w \in \mathbb R^d$. Here, $\sigma$ is the sigmoid function defined by
\begin{eqnarray} 
\sigma(z):=\frac{1}{1+e^{-z}}.
\end{eqnarray}
For the loss function, we use binary cross-entropy (BCE), defined by
\begin{eqnarray}
    \ell(\hat y,y) = -y\log\hat y - (1-y)\log (1-\hat y).
\end{eqnarray}
Let $\widehat w_N$ be obtained via logistic regression fitted on $D'_N$ with ridge regularization parameter $\lambda>0$. Thus, $\hat w$ is the unique\footnote{Unicity is due to strong convexity of objective function.} minimizer of the following objective function
\begin{eqnarray}
L(w) := \frac{1}{N}\sum_{i=1}^N q_i\ell(\sigma(x_i^\top w), y_i') + \frac{\lambda}{2}\|w\|^2.
\label{eq:objective}
\end{eqnarray}
Here $q_i$ is a bit which indicates whether the $i$th training example has survived pruning. The numbers $q=(q_1,\ldots,q_N)$ is called a \emph{pruning strategy}. The corresponding downstream classifier is $\widehat f_N = f_{\widehat w_N}$, where the notation $f_w$ refers to the linear classifier induced by a weights vector $w \in \mathbb R^d$, i.e
\begin{eqnarray}
 f_w(x) := \begin{cases}
1,&\mbox{ if }x^\top w > 0,\\
0,&\mbox{ otherwise.}
\end{cases}
\end{eqnarray}
The test accuracy of the downstream model $\widehat f_N$ is defined by
\begin{eqnarray}
    acc(\widehat f_N) := \mathbb P(\widehat f_N(x) = y),\text{ for a random test point }(x,y) \sim P.
\end{eqnarray}
This quantity will be the main object of our analysis, and we will be interested in how it depends on the corruption level $p$ and the choice of pruning strategy $q$, in the infinite-sample limit $N \to \infty$.

For later reference, we also define an empirical version, namely the accuracy of $\widehat f_N$ evaluated on the clean dataset $D_N$, namely
\begin{eqnarray}
        \widehat{acc}(\widehat f_N) := \frac{1}{|M|}|\{i \in M \mid \widehat f_N(x_i) = y_i\}|,
\end{eqnarray}
where $M := \{i \in [N] \mid q_i = 1\}$ collects the indices of training samples which survive pruning by $q$.

\subsection{A Class of Parametrized Pruning Strategies}
Given hyper-parameters $\phi,\psi \in [0,1]$, we consider a broad class of parametrized pruning strategies with the following properties.
\begin{itemize}
    \item The weights $q_1,\ldots,q_N \in \{0,1\}$ are independent. Thus, whether any training example $(x_i,y_i')$ survives pruning or not is independent of what happens to the other examples. 
    \item The inclusion of an example doesn't depend on the specific labels attributed to this example by the ground-truth labeller $w_*$ or the fake labeller $w_{gen}$, it only depends on whether these labels coincide or not.
   % \item Conditioned on $y_i=k$ and $y'_i = \ell$, the distribution of $q_i$ is Bernoulli with parameter $\phi$ if $k = \ell$ and $\psi$ if $k \ne \ell$. Here, $\psi,\phi \in [0,1]$ are fixed parameters which completely characterize a pruning strategy $q$. % We shall usually write $(\phi,\psi)$ to mean the corresponding strategy $q$.
\end{itemize}
\begin{lemma}
\label{lm:margin-based}
    The above properties are verified when $P$ is a (balanced) Gaussian mixture, the fake data generator is linear model, i.e $y'_i = \operatorname{sign}(x_i^\top w_{gen})$ for some weights vector $w_{gen} \in \mathbb R$, and the pruning strategy is of the form
    \begin{eqnarray}
    q_i = 1[y_i(x_i^\top w_{prune})>0],
    \end{eqnarray}
    for some weights $w_{prune} \in \mathbb R^d$.
\end{lemma}

\yunzhen{Change this lemma to $y'_i \sim \operatorname{sigmoid}(x_i^\top w_{gen})$}

The above properties mean that, for any class labels $k,\ell \in \{0,1\}$, the random variables $(z_{ik\ell})_{i \in [N]}$ defined by $z_{ik\ell}=1[y_i=k,y_i'=\ell,q_i=1]$ are iid with Bernoulli distribution $Bern(p_{k\ell})$, where
\begin{eqnarray}
\label{eq:pkl}
    \begin{split}
p_{k\ell} &= \mathbb P(q_i = 1, y'_i=\ell,y_i=k)\\
&= \mathbb P(q_i=1 \mid y'_i=\ell,y_i=k)\mathbb P(y_i'=\ell \mid y_i=k)\mathbb P(y_i=k)\\
&=
\begin{cases}
    \phi_k(1-p)/2,&\mbox{ if }k=\ell,\\
    \psi_{k\ell}p/2,&\mbox{ else.}
\end{cases}    
    \end{split}
\end{eqnarray}
and the numbers $p$, $\phi_k$ and $\psi_{k\ell}$ are defined by
\begin{eqnarray}
p := \mathbb P(y'_i\ne y_i),\quad \phi_k = \mathbb P(q_i = 1 \mid y'_i=k,y_i=k),\quad \psi_{k\ell}= \mathbb P(q_i = 1 \mid y'_i=\ell,y_i=k).
\end{eqnarray}
Consequently, if $N_{k\ell}$ is the number of training examples that have true label $k$, fake label $\ell$, and survive pruning, then
\begin{eqnarray}
\label{eq:Nkl}
N_{k\ell} := \sum_{i=1}^N z_{ik\ell}
\end{eqnarray}
which is has binomial distribution $Bin(N,p_{k\ell})$. For simplicity of exposition, we shall focus on the case where
\begin{eqnarray}
    \phi_1 = \phi_0 = \phi,\quad \psi_{01}=\psi_{10} = \psi.
\end{eqnarray}
\begin{definition}
\label{df:rlhf-pruning}
Such a pruning strategy will be referred to as an RLHF-type strategy, where RLHF stands for Reinforcement Learning with Human Feedback.

It can be likened to the sense in which the term is classically used, where one assumes access to a strong oracle (e.g a human) who can tell apart bugguous predictions, but can also make mistakes.
\end{definition}
 \ElvisIssue{Link to FC's experiments. Beam-size should map to some value of $(\phi,\psi)$.} 
 \begin{remark}
    Note that the parametrization $(\phi,\psi)$ and $(p_{00},p_{11})$ describe the same RLHF-type policy via the following bijective transformation.
    \begin{align}
        p_{00} &= p_{11} = (1-p)\phi/2,\quad p_{01}=p_{10} = 
 p \psi /2.
    \end{align}
\end{remark}

\subsection{Examples}
Let us present some notable examples of pruning RLHF-type pruning strategies (Definition \ref{df:rlhf-pruning}).

\paragraph{No Pruning.} The case $(\phi,\psi) = (1,1)$ corresponds to no pruning, i.e the entire training dataset is used. This is reminiscent of classical machine learning. \julia{hahaha. I like ``reminiscent". }
     \paragraph{Pure RLHF.} The case $(\phi,\psi) = (1,0)$. The pruning strategy only keeps indices corresponding to examples in the dataset which have correct label (all corrupted labels discarded). 

\paragraph{Margin-Based Pruning.} Let $w_{prune} \in \mathbb R^d$, and consider the pruning strategy defined by
    \begin{eqnarray}
    \label{eq:margin-based}
    q_i = 1[y_i(x_i^\top w_{prune})>0].
    \end{eqnarray}
    % where $z'_i := 2y_i'-1$. Note that $z'_ix_i^\top w$ is the margin of $(x_i,y_i')$ w.r.t to the decision boundary of the linear model $f_w(x) := \mathrm{sign}(x^\top w)$. In Lemma \ref{lm:margin-based}, we show that for symmetric classification problem (refer to Definition \ref{df:symmetric}), such a pruning scheme is in fact an instance of an RLHF-type pruning scheme with parameters $\phi=P_1(w,m)$ and $\psi=P_0(w,m)$, where the $P_k(w,m)$' are as defined in \eqref{eq:Pk}.
    This pruning strategy simplify filters out all examples on which it disagrees on the assigned label. 

\bbb{
For Gaussian mixture distribution $P$ with isotropic covariance, we have
$$
p_{00} = p_{11} = \mathbb P(x^\top w_p > 0,\, x^\top w_g > 0 \mid y=1)\mathbb P(y=1) = \mathbb P(z_p >-\mu^\top w_p,\,z_g >-\mu^\top w_g)/2,
$$
where $(x,y) \sim P$, so that the distribution of $x$ conditioned on $y=1$ is $N(\mu, \Sigma)$ with $\Sigma=I_d$; $z_g:=z^\top w_g$ and $z_p:=z^\top w_p$, for $z \sim N(0,\Sigma)$.
Now, assume WLOG that $\|w_g\|=\|w_p\|=1$, and observe that $(z_g,z_p)$ is bivariate normal with variance $\sigma^2=1$ and correlation coefficient $\rho=w_p^\top w_g$. The joint pdf is thus
$$
f(u,v) = \frac{1}{2\pi\Delta}e^{-\frac{1}{2\Delta^2}(u^2+v^2-2\rho u v)} = \frac{1}{\sqrt{2\pi\Delta^2}}e^{-\frac{1}{2\Delta^2}(v-\rho u)^2}\frac{1}{\sqrt{2\pi}}e^{-u^2/2},
$$
where $\Delta=\sqrt{1-\rho^2}$. We deduce that
\begin{align*}
   2 p_{00} &= \int_{-\mu^\top w_g}^\infty \left(\int_{-\mu^\top w_p}^\infty \frac{1}{\sqrt{2\pi\Delta^2}}e^{-\frac{1}{2\Delta^2}(v-\rho u)^2}\mathrm dv\right)\varphi(u)\mathrm du\\
    &= \int_{-\mu^\top w_g}^\infty\Phi\left(\frac{\rho u+\mu^\top w_p}{\Delta}\right)\varphi(u)\mathrm du\\
    &= \int_0^\infty \Phi\left(\frac{\rho (u + \mu^\top w_g) + \mu^\top w_p}{\Delta}\right)\varphi(u+\mu^\top w_g)\mathrm du.
\end{align*}
One can derive similar expressions for $p_{01}=p_{10}$,
namely
\begin{align*}
2p_{01} = \int_0^\infty \Phi\left(\frac{\rho (u - \mu^\top w_g) - \mu^\top w_p}{\Delta}\right)\varphi(u-\mu^\top w_g)\mathrm du.
\end{align*}
}

% The following theorem will be useful in the sequel
% \begin{theorem}
%     For the case of margin-based pruning, it holds that
%     \begin{align}
%     p &= \theta_{gen},\\
%         p_{00} &= p_{11} = \frac{1}{2} - \frac{1}{4\pi}(\theta_{gen} 
% + \theta_{prune} + \theta_{gp}),\\
% p_{01} &= p_{10}  = \frac{1}{4\pi}(\theta_{gen} + \theta_{p} - \theta_{gp}).
%     \end{align}
% where $\theta_{gen} \in [0,\pi]$ is the angle between $w_{gen}$ and $w_*$; $\theta_{prune} \in [0,\pi]$ is the angle between $w_{prune}$ and $w_*$; $\theta_{gp} \in [0,\pi]$ is the angle between $w_{gen}$ and $w_{prune}$.

% In particular, the following hold.

% (A) \textbf{Perfect Generator.} If $w_{gen}=w_*$, then
%     $p = 1/2,\, p_{00} = p_{11} = (1-\theta_{prune})/2,\, p_{01}=p_{10}=0$.
    
% (B) \textbf{Perfect Pruner.} If $w_{prune}=w_*$, then
% $p_{00} = p_{11}=(1-p)/2,\, p_{01}=p_{10}=0$.

% (C) \textbf{No Pruning.} If $w_{prune}=w_{gen}$
%     $p = 1/2,\, p_{00} = p_{11} = (1-p)/2,\, p_{01} = p/2$.
% \end{theorem} 
% \begin{proof}
%     $(x^\top w_{gen},x^\top w_{prune}, x^\top w_{prune})$ have a trivariate Gaussian distr;
% \end{proof}
% As we shall see, the downstream test accuracy (on clean data!) exhibits a sharp phase-transition across the manifold $p_{00}=p_{01}$, i.e $\theta_{gen}+\theta_{prune} = \pi$, or equivalently, $\theta_{prune} = (1-p)\pi$.
% \begin{mdframed}
% \textbf{Criticality.} The test accuracy is $100\%$ for $p < 
%  (1 - \epsilon)p_{crit}$ and $0\%$ for $p > (1 +\epsilon)p_{crit}$,
% where
% \begin{eqnarray}
% p_{crit} := 1-\theta_{prune}/\pi,
% \end{eqnarray}
% i.e test accuracy of the pruner (seen as a classifier).
% In particular, for the case of no-pruning (here corresponding to $w_{prune} = w_{gen})$, one has $\theta_{prune} = \theta_{gen} = 1-p$, and so $p_{crit} = 1/2$, which is not surprising. For smaller values of $\theta_{prune}$ (i.e $w_{prune}$ close to the ground-truth $w_*$), this breakpoint $p_{crit}$ becomes bigger, reflecting a higher tolerance to fake data.  \ElvisIssue{This perhaps provides an indirect explanation for some of the results of FC. Please check!}
% \end{mdframed}
 

% \subsection{A Generalization}
%   We can easily extend the definition of RLHF-type pruning strategies (Definition \ref{df:rlhf-pruning}) by considering a more general form for the $p_{k\ell}$'s appearing in \eqref{eq:pkl}, viz
%     \begin{eqnarray}
%         p_{k\ell} = \begin{cases}
%             (1-p)\phi_k/2,&\mbox{ if }k = \ell,\\
%             p\psi_{k\ell}/2,&\mbox{ if }k \ne \ell,
%         \end{cases}
%     \end{eqnarray}
%     for some scalars $\phi_0,\phi_1,\psi_{01},\psi_{10}\in [0,1]$. For simplicity of exposition, we only consider the special case above where $\phi_k=\phi$ and $\psi_{k\ell}=\psi$ for all $k,\ell$, giving \eqref{eq:pkl}. With this modification, every margin-based pruning strategy $(w,m)$ on a binary classification problem (symmetric or not, in the sense of Definition \ref{df:symmetric}) is a generalized RLHF-type pruning strategy with parameters
%     \begin{eqnarray}
%         \phi_{00} = P_0(-w,m),\quad \phi_{11}=P_1(w,m),\quad \psi_{01}=P_0(w,m),\quad \phi_{10}=P_1(-w,m),
%     \end{eqnarray}
%     where the $P_k(w,m)$'s are as defined in \eqref{eq:Pk}.

\subsection{Performance Bounds for Models Trained with RLHF Pruning}
    \begin{figure}[!htb]
    \centering
        \includegraphics[width=.45\textwidth]{RLHF.png}
        \includegraphics[width=.43\textwidth]{thresholds.png}
    % \includegraphics[width=.45\textwidth]
    % {prune.png}
   \caption{\textbf{Empirical Confirmation of Theorem \ref{thm:main}.} Comparing the breakdown points of different models. Here, the task is classifying a Gaussian mixture, with infinite training samples from datasets generated from a model with classification error rate $p$ (x-axis). Notice the sharp phrase-transitions where the model suddenly switches from perfect accuracy to worse-than-chance, a phenomenon predicted by Theorem \ref{thm:main}. % \textbf{Top Right.} "SD" stands for self-distillation, and "xn" means iterative self-distilling the same model $n$ times. Notice how a model pruning with a teacher's margin is already stronger than a few distillations (here it seems to actually matches double-distillation), and much stronger than the original student. Also notice how repeated self-distillation approaches RLHF. 
    \textbf{Left.} Performance of RLHF-type pruning strategies with different values of the  hyper-parameters $(\phi,\psi)$. Recall that the case $\psi/\phi=1$ corresponds to no pruning, while $\psi/\phi=0$ corresponds to pure RLHF. \textbf{Right.} Comparing $p_{up}$, approximated with $\sup\{p \mid acc(\widehat f_N) \ge 90\%\}$ (computed empirically), against the analytic estimate $p^-_\star(t)$ given in \ref{thm:main} (for $t=0.1$). Again, the results are in excellent agreement with the predictions of Theorem \ref{thm:main}. \yunzhen{Do we need these two figures in the main paper?}
    % Even for $p > 1/2$, notice how the models with $\psi/\phi<1$ still continue to perhaps above chance level ($50\%$ accuracy). % \textbf{Bottom.} Comparing with margin-based pruning strategies. Again, notice the sharp phrase-transitions predicted by Theorem \ref{thm:main}.
    }
    \label{fig:curves}
\end{figure}
The following is one of our main results (proved in the appendix).
\begin{theorem}
\label{thm:main}
Suppose Condition \ref{cond:main} is in order. Fix $\phi,\psi,t \in (0,1)$ and define $p^\pm_\star(t) \in (0,1)$ by
\begin{eqnarray}
    p^-_\star(t) := \frac{1 - t}{1 - t + (1 + t)\psi/\phi},\quad p^+_\star:=\frac{1 + t}{1 + t + (1 - t)\psi/\phi}
    \label{eq:threshold}
\end{eqnarray}
If $p < p^-_\star(t)$, then the limit $N \to \infty$ it holds w.p $1-o(1)$  that the $acc(\widehat f_N) = 100\%$ for a downstream model $\widehat f_N$ trained on data from  a generator with error rate $p$ pruned with an RLHF-type strategy  with parameters $(\phi,\psi)$.

On the other hand, if $p > p^+_\star$, then the limit $N \to \infty$ it holds w.p $1-o(1)$  that the $acc(\widehat f_N) = 0\%$ for a downstream model $\widehat f_N$.

Thus, there is a sharp phase-transition around the corruption level $p_\star := 1/(1+\psi/\phi)$: as $p$ is increased past level $p_\star$, the downstream model $\widehat f_N$ abruptly switches from being perfectly accurate, to perfectly inaccurate!
\end{theorem}
See Figure \ref{fig:curves} for an empirical illustration of the theorem.

The thresholds $p^\pm_\star(t)$ appearing in the above theorem is are proxies for the so-called \emph{breakdown points} $p_{up} \ge p_{down}$ defined by
\begin{align}
    p_{up} &= \inf\left\{p \in [0,1] \,\big|\, acc(\widehat f_N) \overset{a.s}\to 0\%\text{ in the limit }N \to \infty\right\},\\
        p_{down} &= \sup\left\{p \in [0,1] \,\big|\, acc(\widehat f_N) \overset{a.s}\to 100\%\text{ in the limit }N \to \infty\right\}.
\end{align}
Theorem \ref{thm:main} implies $p_{down} \ge p^-_\star(t)$ and $p_{up} \le p^+_\star(t)$ for all $t \in (0,1)$. Consequently,
\begin{corollary}
    Under the hypotheses of Theorem \ref{thm:main}, it holds that $p_{up} = p_{down}$.
\end{corollary}

\subsection{Some Consequences of Theorem \ref{thm:main}}
We now present some illustrious applications of Theorem \ref{thm:main}. These examples are empirically confirmed in Figure \ref{fig:curves}.


\paragraph{No Pruning.}
Here, we have $\psi/\phi=1$ and so the downstream model achieves $100\%$ accuracy for all values of corruption parameter $p$ up to the proxy  breakdown point predicted by Theorem \ref{thm:main} is then $p^-_\star = 1/2-t/2$.

\paragraph{Pure RLHF.} For this scenario, $\psi/\phi=0$ and  so Theorem \ref{thm:main} predicts that the downstream model $\widehat f_N$ achieves $100\%$ accuracy for all values of corruption parameter $p$ up to the breakdown point $p^-_\star = 1$. This is perhaps not so surprising in hindsight. The point is that even for moderately large values of $\psi/\phi$, the proxy breakdown point $p^-_\star$ given in \eqref{eq:threshold} can still be quite close to $1$.

\paragraph{Margin-Based Pruning.}
Consider Gaussian mixture data with means $\pm \mu$, and consider a margin-based pruning strategy in Lemma \ref{lm:margin-based}. It is clear that $\phi$ and $\psi$ on depend on all the 3 angles between the set of vectors $\{w_*,w_{gen},w_{prune}\}$, with $w_*=\mu$. \yunzhen{One might use a $w_{prune}$ with similar or better performance compared to $w_{gen}$; however, the selected data may not show improvement beyond $w_{gen}$. This explains why using LLaMA3 does not enhance selection.}

\subsection{Sketch of Proof of Theorem \ref{thm:main}}
The proof is based on the following representation (refer to Proposition \ref{prop:acc}) of the accuracy of the downstream classifier $\widehat f_N$ evaluated on the the clean training dataset $D_N$, namely
\begin{eqnarray}
\widehat{acc}(\widehat f_N) = \frac{N_{11}1_{\overline A < 1/2} + N_{00} 1_{\overline D < 1/2} + N_{10}1_{\overline B > 1/2} + N_{01} 1_{\overline C > 1/2}}{N_{11} + N_{00} + N_{10} + N_{01}},
\end{eqnarray}
for some random some random variables $\overline A,\overline B,\overline C,\overline D \in (0,1)$ which depend on the $N_{k\ell}$'s defined in \eqref{eq:Nkl}. By classical results in learning theory (e.g., see Kakade, Sridharan, and Tewari (2008) "On the Complexity of Linear Prediction: Risk Bounds, Margin Bounds, and Regularization"), we know that the gap to the population version (test accuracy) $acc(\widehat f_N)$ shrinks to zero at rate $O(1/N)$, and so since the claim in Theorem \ref{thm:main} is made only in the limit $N \to \infty$, we are good.  

Next, in Proposition \ref{prop:symmetric-case} and Proposition  \ref{prop:skewed-case}, necessary and sufficient conditions are established to ensure $\overline A,\overline D < 1/2$ and $\overline B,\overline C > 1/2$, and therefore $\widehat{acc}(\widehat f_N) = 100\%$. These conditions are given explicitly in terms of the $N_{k\ell}$'s. Finally, in Proposition \ref{prop:concentration}, concentration of measure is used to control the $N_{k\ell}$'s, and present the aforementioned conditions in terms of the $p_{k\ell}$'s defined in \eqref{eq:pkl}, and therefore in terms of $p$, $\phi$, and $\psi$ alone, giving condition \eqref{eq:threshold}.
\label{prop:acc-informal}

